A Risk Decomposition Framework for Pre-Hoc Fine-Tuning Prediction

The high cost of fine-tuning LLMs poses a significant economic barrier; pre-hoc performance prediction offers a critical solution to substantially reduce this expense. However, the theoretical limits of pre-hoc performance prediction remain unexplored. We formulate it as a stochastic estimation problem under information constraints, decomposing prediction risk into two components: an intrinsic limit (static data-model compatibility) and a reducible optimization variance. We prove that optimization variance admits a necessary lower bound on its decay rate, implying fundamental constraints on how quickly uncertainty dissipates, regardless of the predictor used. Based on these dynamics, we derive a budget-optimal probing principle and introduce a predictability phase diagram that organizes tasks into three distinct regimes: Static-Sufficient, Dynamic-Critical, and Noise-Dominant. Extensive experiments on synthetic and real-world benchmarks validate these theoretical regimes and demonstrate the efficiency of our probing strategy.

==> misc/commands.tex <==
%!TEX root = ../main.tex
\newcommand{\eat}[1]{}
\usepackage{placeins}
\usepackage{balance}
\usepackage{times}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amsmath}
% \usepackage{amssymb}
\usepackage{colortbl}
\usepackage{epsfig}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{bbm}
% \usepackage{cite}
\usepackage{comment}
\usepackage{booktabs}
\usepackage{multirow}
%\usepackage[dvipsnames]{xcolor}
\usepackage{framed}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{caption}
\setlength{\intextsep}{4pt}   % 图与上下正文之间的竖直间距（越小越紧凑）
\usepackage{booktabs}
\usepackage[table]{xcolor}
\usepackage{subcaption} % 新增

\setlength{\columnsep}{10pt}  % 图与环绕文字的水平间距
\captionsetup{font=small, labelfont=bf, skip=2pt}
\usepackage{circledsteps}
\usepackage[utf8]{inputenc}
\usepackage{microtype}
\usepackage{inconsolata}
\usepackage[colorlinks=true, linkcolor=black, urlcolor=magenta, citecolor=black]{hyperref}
\usepackage{float}
\newtheorem{example}{Example}
\usepackage{chngcntr}
%\usepackage{algorithmicx}
% \usepackage{algorithm} 
\usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{algpseudocode}
% \usepackage[algo2e]{algorithm2e} 

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\Output{\item[\algorithmicoutput]}

\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}
\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\usepackage{lineno}
\renewcommand\linenumberfont{\normalfont\tiny\sffamily} % 让行号小一些（可选）


\newcommand{\red}[1]{\textcolor{red}{#1}}
\definecolor{green}{RGB}{0,128,0}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\definecolor{yellow}{RGB}{255,200,18}
\newcommand{\yellow}[1]{\textcolor{yellow}{#1}}
\newcommand{\pink}[1]{\textcolor{magenta}{#1}}
\newcommand{\violet}[1]{\textcolor{violet}{#1}}

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\newcommand{\add}[1]{\textcolor{blue}{{#1}}}
\newcommand{\revised}[1]{\textcolor{blue}{{#1}}}
\newcommand{\rewrite}[1]{\textcolor{gray}{{#1}}}
\newcommand{\notice}[1]{\textcolor{red}{{#1}}}

% \sloppy
\newcommand{\rtable}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\ratt}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\at}[1]{\protect\ensuremath{\mathsf{#1}}}
\newcommand{\att}[1]{\textbf{\texttt{#1}}}
\newcommand{\myhrule}{\rule[.5pt]{\hsize}{.5pt}}
\newcommand{\oneurl}[1]{\texttt{#1}}
\newcommand{\tabstrut}{\rule{0pt}{4pt}\vspace{-0.1in}}
\newcommand{\stab}{\vspace{1.2ex}\noindent}
\newcommand{\sstab}{\rule{0pt}{8pt}\\[-2.2ex]}

\newcommand{\exa}[2]{{\tt\begin{tabbing}\hspace{#1}\=\+\kill #2\end{tabbing}}}

\newcommand{\match}{\rightleftharpoons}


\newcommand{\true}{\kw{true}}
\newcommand{\kop}{\kw{op}}
\newcommand{\nil}{\kw{nil}}
\newcommand{\Op}{\kw{Op}}

\newcommand{\la}{\leftarrow}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\mat}[2]{{\begin{tabbing}\hspace{#1}\=\+\kill #2\end{tabbing}}}
\newcommand{\m}{\hspace{0.05in}}
\newcommand{\ls}{\hspace{0.1in}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\beqn}{\begin{eqnarray*}}
\newcommand{\eeqn}{\end{eqnarray*}}
\newcommand{\card}[1]{\mid\! #1\!\mid}
\newcommand{\fth}{\hfill $\Box$}
\newcommand{\Sm}[1]{\displaystyle{\sum_{#1}}}
\newcommand{\stitle}[1]{\stab\noindent{\bf #1}}
\newcommand{\etitle}[1]{\vspace{1mm}\noindent{\underline{\em #1}}}
\newcommand{\ie}{{\em i.e.,}\xspace}
\newcommand{\eg}{{\em e.g.,}\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\xspace}
\newcommand{\aka}{\emph{a.k.a.}\xspace}
\newcommand{\kwlog}{\emph{w.l.o.g.}\xspace}

\newcommand{\eop}{\hspace*{\fill}\mbox{$\Box$}}     % End of proof

%% Only used in the template examples. You can remove these lines.
\usepackage{tabu}                      % only used for the table example
\usepackage{booktabs}                  % only used for the table example
\usepackage{lipsum}                    % used to generate placeholder text
\usepackage{mwe}                       % used to generate placeholder figures

%% We encourage the use of mathptmx for consistent usage of times font
%% throughout the proceedings. However, if you encounter conflicts
%% with other math-related packages, you may want to disable it.
% \usepackage{mathptmx}                  % use matching math font

\usepackage{listings}
\usepackage{tcolorbox}
\usepackage{pifont}
\usepackage{tikz}
\usepackage{enumitem}
\usepackage{natbib}
\usepackage{utfsym} % For checkmarks and cross symbols
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc} 

\usetikzlibrary{shapes,snakes}
\usetikzlibrary{calc}

\definecolor{shadecolor}{RGB}{220,220,220}
\newcommand{\mybox}[1]{\vspace{1.5ex}\par\noindent\colorbox{shadecolor}
	{\parbox{\dimexpr\columnwidth-2\fboxsep\relax}{#1}}\vspace{1.5ex}}
	

\tikzstyle{mybox} = [draw=black, fill=black!5, thick,
    rectangle, rounded corners, inner sep=2pt, inner ysep=8pt]
\tikzstyle{fancytitle} =[fill=black, text=white]


%\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%		\node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

% Project level macros
\newcommand{\sys}{\textbf{\textsc{TuneAhead}}\xspace}
% \newcommand{\cbench}{{CommonSense}\xspace}
% \newcommand{\ebench}{{ETL}\xspace}
% \newcommand{\scbench}{{Science}\xspace}
\newcommand{\EnableAppendixFloatNumbering}{%
  \counterwithin{figure}{section}%
  \counterwithin{table}{section}%
  \renewcommand{\thefigure}{\thesection.\arabic{figure}}%
  \renewcommand{\thetable}{\thesection.\arabic{table}}%
  \setcounter{figure}{0}%
  \setcounter{table}{0}%
}
\apptocmd{\appendix}{\EnableAppendixFloatNumbering}{}{}

% Reviewer level macros
\newcommand{\yuyu}[1]{\textcolor{blue}{{\bf$^{Yuyu}$[#1]}}}
\newcommand{\nan}[1]{\textcolor{red}{{\bf$^{Nan}$[#1]}}}
\newcommand{\yuxiang}[1]{\textcolor{teal}{{\bf$^{yuxiang}$[#1]}}}


